LTE Standard-Compliant D2D Communication: Software-defined Radio Implementation and Evaluation

In this paper, we describe the design and implementation of D2D communication functionality for LTE. To our knowledge, this is the first such implementation that is compliant with the LTE Release 12 standard. In this paper, we design and demonstrate an experiment on mode selection between infrastructure mode and D2D communication mode in LTE networks. We implement our system on a software-defined radio SDR testbed, augmenting the open-source LTE eNodeB and UE implementation provided by the srsLTE software suite. Our measurements demonstrate the cell extension capabilities of D2D and quantify the SNR and throughput obtained by a subscriber when directly served by the eNodeB and when provided connectivity through the relay UE. Our implementation of sidelink, relaying, and mode selection functionality enables experimentation and prototyping of D2D communication that can assist in standardization, research, and development.

==> LTE Standard-Compliant D2D Communication%3A Software-defined Radio Implementation and Evaluation/sections/Additional_Contribution.tex <==
\section{Controller GUI for dynamic parameter settings}
\label{sec:Additional_Contribution}

We also built a user interface that allows experimenters to change the radio parameters, such as frequency, gain, and \ac{MCS}, on the fly for the eNodeB, relay \ac{UE} and remote \ac{UE}. We used the \textit{pThread} library in C to create threads that receive external commands from users and translate them into parameters settings in the srsLTE implementation. We used the GTK+ 3.0 library in C to implement the GUIs, and we implemented the communication between the \ac{GUI} and our \ac{LTE} software (based on a client-server scheme) using Linux socket interprocess communication libraries. The elements of our implementation include: 

%we develop the controllers with GUIs to connect with the Application Programming Interface (API) of the downlink/sidelink software for flexible control.

\subsubsection{Controller GUI for eNodeB}
This eNodeB controller \ac{GUI} (shown in Fig.~\ref{fig:enodeb_GUI}) has the functionality to change frequency, gain, \ac{PRBs}, amplitude, \ac{MCS} index and cell ID.  

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/enodeb_GUI}  %trim= l b r t
	\caption{Controller GUI for eNodeB.}
	\label{fig:enodeb_GUI}
\end{figure}


\subsubsection{Controller GUI for relay UE}

The controller \ac{GUI} for the relay \ac{UE}, shown in Fig.~\ref{fig:relay_GUI}, provides an interface for the downlink receiver and the sidelink transmitter, as the relay UE performs both functions at the same time. For the downlink receiver, the experimenter can change frequency, gain, and \ac{RNTI}. For the sidelink transmitter, the experimenter can change frequency, gain, amplitude, \ac{PRBs} and \ac{MCS} Index. This GUI has two different socket port options to connect to the \ac{LTE} software, so that the downlink and sidelink parameters are controlled separately via different Linux socket ports, providing additional flexibility to the experimenter. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/relay_GUI}  %trim= l b r t
	\caption{Controller GUI for the relay UE, showing the control of both downlink and sidelink parameters.}
	\label{fig:relay_GUI}
\end{figure}

\subsubsection{Controller GUI for remote UE}

The controller \ac{GUI} for the remote \ac{UE} comprises three \ac{GUI} windows. The first \ac{GUI} acts as the controller through which the mode selection between downlink and sidelink can be performed (shown in Fig.~\ref{fig:remote_controller}). 
%This Remote controller \ac{GUI} has two buttons for selecting the mode. 
If the experimenter selects the downlink mode, the \ac{LTE} radio software for the downlink automatically boots up and the \ac{GUI} for the downlink opens up (as shown in Fig.~\ref{fig:remote_downlink_GUI}), and similarly for the sidelink mode (as shown in Fig.~\ref{fig:remote_sidelink_GUI}. The parameters which the experimenter can control through downlink or sidelink \ac{GUI} are similar to those of the downlink GUI for the relay \ac{UE}. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/remote_controller}  %trim= l b r t
	\caption{Controller GUI for the remote UE: mode selection.}
	\label{fig:remote_controller}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/remote_downlink_GUI}  %trim= l b r t
	\caption{Controller GUI for the remote UE using the downlink.}
	\label{fig:remote_downlink_GUI}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/remote_sidelink_GUI}  %trim= l b r t
	\caption{Controller GUI for the remote UE using the sidelink.}
	\label{fig:remote_sidelink_GUI}
\end{figure}

==> LTE Standard-Compliant D2D Communication%3A Software-defined Radio Implementation and Evaluation/sections/Implementation.tex <==
\section{Design and Implementation}
\label{sec:Implementation}

As described in the previous section, our design and implementation focuses on the LTE sidelink and relay functionality. In this section, we outline the major technical challenges in implementing this functionality. The first challenge is to develop the sidelink PHY layer data transmission channels, which adopt a \ac{SC-FDMA} waveform, according to the \ac{LTE} standard. The second challenge is to build the relay functionality for the UE. The third challenge is to design the mode selection functionality in the remote UE to establish either a sidelink (with the relay UE) or a downlink connection (with the eNodeB). 
 

\subsection{Implementation of \ac{PSSCH} with \ac{SC-FDMA}}

The \ac{PSSCH} is the \ac{PHY} channel for data transmission on the sidelink. 
%We implement the \ac{PSSCH} based on the open-source srsLTE software library whose uplink and downlink modules are available.
According to the \ac{3GPP} \ac{LTE} standard Release 12, the PSSCH must use \ac{SC-FDMA} for data transmission. The main  difference in implementation between \ac{SC-FDMA} and \ac{OFDM} (which is used in the downlink) is that an additional \ac{DFT} is needed in the transmitter and an additional \ac{IDFT} is needed in the receiver, as shown in Fig.~\ref{fig:sc_fdma}. We implement the \ac{PSSCH} by inserting the \ac{DFT} and \ac{IDFT} modules, available at the FFTW3 and srsLTE software library, into the \ac{OFDM} radio \ac{DSP} chain for the \ac{PSSCH}. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.5\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/sc_fdma}  %trim= l b r t
	\caption{Block diagram of SC-FDMA transmitter (Tx) and receiver (Rx).}
	\label{fig:sc_fdma}
\end{figure}

A \ac{PSCCH} is also needed for accomplishing the functionality of \ac{PSSCH}. In our sidelink implementation, three symbols per subframe are allocated for the \ac{PSCCH}, and \ac{SCI} is included in these symbols.
%\ac{SCI} is utilized by the \ac{PSSCH} to transmit the control information simultaneously with data  in order to encode/decode the data successfully. According to the \ac{3GPP} \ac{LTE} standard, 
The \ac{SCI} may include information on the \ac{MCS}, a group destination identifier, the resource block assignment and hopping resource allocation, a frequency hopping flag, etc. In our implementation we include minimum functionality for the \ac{PSCCH}, supporting flexible \ac{MCS} selection by the sidelink controller (to be described in the following sections). For the moment, we 
%have implemented only one sidelink transmitter \ac{UE} and one sidelink receiver \ac{UE} as a proof-of-concept. Therefore in our implementation we 
assign the entire set of resource blocks in the frequency channel of the sidelink to a single pair of \acp{UE}. 
%We plan to implement the frequency hopping and other functions in \ac{PSCCH} as our future work. Besides, for more intelligent use cases of sidelink that involves other sidelink \ac{PHY} channels for more sophisticated signaling and user discovery, e.g. \ac{PSDCH}, etc, we also plan to design and implement them in our future work.




\subsection{Implementation of relay functionality in the UE}

The relay \ac{UE} is called upon to relay the data received in the downlink to the remote UE, communicating over the sidelink. In order to run the downlink and sidelink in parallel, we create two different threads, which individually perform the two sets of operations without interrupting each other. The internal functionality of the relay \ac{UE} is shown in Fig.~\ref{fig:block_relay_UE}. A \ac{UE} must  establish the link with the eNodeB, first searching for beaconing signals periodically transmitted by the base station (in the figure, this process is referred to as a cell search). After the downlink is established, the \ac{UE} must decode the \ac{PSS} and \ac{MIB} signals to synchronize with the eNodeB. Then, it decodes the \ac{PDCCH} and the \ac{PDSCH} signals to receive data, which subsequently needs to be forwarded to the remote \ac{UE} over the sidelink. This data is then transmitted over the \ac{PSSCH} using \ac{SC-FDMA}. The \ac{PSSS} signal is also generated simultaneously, for synchronization between  two UEs that have established a sidelink. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.5\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/block_relay_UE}  %trim= l b r t
	\caption{Block diagram of the relay UE.}
	\label{fig:block_relay_UE}
\end{figure}

\subsection{Implementation of mode switching}

We implement functionality for the remote \ac{UE} that enables it to switch between sidelink and downlink modes of operation in real time. A controller is needed to perform this mode switching with minimum latency. We implement our controller with two separate threads: one calls up the \ac{OFDM} receiver for the downlink and the other one calls up the receiver for the sidelink. The threads run the individual Linux bash commands which can boot either the downlink or sidelink program automatically. For experimental purposes, we build a \ac{GUI} on top of this controller that can be used by an experimenter to manually switch between operation modes, as further described in  section~\ref{sec:Additional_Contribution}.





==> LTE Standard-Compliant D2D Communication%3A Software-defined Radio Implementation and Evaluation/sections/Measurement_Results.tex <==
\section{Experimental Results}
\label{sec:Results}

To verify the correct operation of the solutions described above, and to collect performance measurement results, we have set up an experiment as shown in Fig.~\ref{fig:testbed_set_up}. The figure shows the eNodeB on the left hand side, a \ac{UE} that serves as a relay in the middle, and the remote UE on the right hand side. For the experiments reported here, we adopted the \ac{USRP} reconfigurable radio model B210 and the \ac{UHD} interface. The \ac{USRP} B210 hardware supports a 30.72 MHz clock, matching \ac{LTE} sampling frequencies and enabling the decoding of signals from live \ac{LTE} base stations. Our experiment consists of three \ac{USRP} B210 and three laptops running srsLTE software, extended with our sidelink and relay implementation. Each \ac{USRP} connects to a different laptop through a \ac{UHD} driver and USB 3.0. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/testbed_set_up}  %trim= l b r t
	\caption{Experimental set-up.}
    	\label{fig:testbed_set_up}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/Results_scenario}  %trim= l b r t
	\caption{Measurement scenario.}
    	\label{fig:Results_Scenario}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/Measurement_ResultsPNG}  %trim= l b r t
	\caption{Measurement Setup.}
    	\label{fig:measurement_setup}
\end{figure}



In our measurements we maintain the locations of eNodeB and relay \ac{UE} fixed and move the remote UE, starting from the position of the eNodeB, towards the edge of the cell
%. To start with a basic measurement, we use a 1-dimension map to simplify the geolocations of the eNodeB and UEs, 
as depicted in Fig.~\ref{fig:Results_Scenario}.
A photograph of the measurement set-up is shown in Fig.~\ref{fig:measurement_setup}.
The measurements focus on how the \ac{SNR} and throughput vary with the position of the remote \ac{UE}. In the tests, a downlink signal is transmitted from the eNodeB to the remote \ac{UE} and sidelink signal is transmitted from the relay \ac{UE} to the remote \ac{UE}. To accommodate the range restrictions of the RF hardware and the space available in the laboratory where the experiments took place, we fixed the transmitter gain for the eNodeB at 55 dB, yielding a cell boundary at approximately 256 cm.
%In order to create a scenario that is close to the real world while fitting the equipment in the size of our testbed room and the transmitter gain of the eNodeB is fixed at 55 dB in order to set the cell edge to be 256cm.

%We have performed two measurements, based on \ac{SNR} and throughput respectively, so that two mode selection methods can be applied based on these measurements. 
The following subsections describe the measurement results.

\subsection{SNR measurements and mode selection}

Fig.~\ref{fig:SNR_vs_Distance_40} shows the average \ac{SNR} as a function of distance, measured from the location of the eNodeB to the remote UE, for both the sidelink (orange curve) and downlink (blue curve), when the transmitter gain of the sidelink is fixed at 40 dB. (This is lower than the transmitter gain for the downlink because the relay \ac{UE} is supposed to have lower power consumption for transmission and lower coverage than an eNodeB.) 
It is clear that, up to around 160 cm from the eNodeB, the downlink offers superior SNR to the sidelink; past that point, establishing a sidelink to a relay UE provides an SNR advantage. Beyond a distance of around 240 cm from the eNodeB, the only option available to the remote UE is to set up a sidelink: this illustrates the range extension capabilities of D2D.
%The remote \ac{UE} is moved from 0 cm to 280 cm and the \ac{SNR} from downlink and sidelink are compared. 
%From the graph, we can see that if the remote \ac{UE} is moved from the eNodeB to the cell boundary and beyond, the remote \ac{UE} should do downlink till it reaches around 160 cm after which the \ac{SNR} through sidelink (relay) gets better. Now at 160 cm the remote \ac{UE} should perform sidelink. At 256 cm, which is the cell edge i.e. after this point downlink does not work, the remote \ac{UE} has to perform sidelink to get cellular coverage. This proves that \ac{D2D} helps in increasing the coverage.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/SNR_vs_Distance_pic1}  %trim= l b r t
	\caption{SNR vs. distance for 40 dB sidelink transmitter gain.}
    	\label{fig:SNR_vs_Distance_40}
\end{figure}

Fig.~\ref{fig:SNR_vs_Distance_30} shows  similar results of average \ac{SNR} versus distance, but in this case the sidelink transmitter gain has been set to 30 dB. We can see that around 180 cm is the switching point from downlink to sidelink, if the objective is to maximize SNR. We can also see that the \ac{SNR} for the sidelink is lower than that reported in Fig.~\ref{fig:SNR_vs_Distance_40}, and the effective range extension is also reduced, reflecting the lower setting for the sidelink gain.
%in comparison to \ac{SNR} when the gain was 40 dB for sidelink. But the \ac{SNR} is still higher in comparison to downlink, suggesting that remote \ac{UE} should switch to sidelink after 180 cm. The coverage of sidelink at 30 dB gain gets reduced compared to 40 dB gain, since at 30dB the sidelink transmitter is able to transmit shorter distance.

Each point in Fig.~\ref{fig:SNR_vs_Distance_40} and Fig.~\ref{fig:SNR_vs_Distance_30} is the average of 1000 collected measurements. 
%We have measured 1000 samples for each distance. The further statistical analysis regarding 
We also report the standard deviation, the width of the 95\% confidence internal, minimum, and maximum SNR in the Tables \ref{table:1}, \ref{table:2}, and \ref{table:3}. 
%The confidence level we assume is 95\%. 
Statistical analysis reveals that, for each value of distance, the \ac{SNR} varies very little and hence we have very tight confidence intervals.
%small standard deviation. Furthermore, With a big population of samples we have got very small confidence interval, They are too small to be visible if we put them in the aforementioned pictures.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/SNR_vs_Distance_pic2}  %trim= l b r t
	\caption{SNR vs. distance for 30 dB sidelink transmitter gain.}
    	\label{fig:SNR_vs_Distance_30}
\end{figure}

\begin{table}[ht]
\caption{Statistical analysis of the SNR for the sidelink, at 30 dB transmitter gain.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \textbf{Distance} & \textbf{Average} & \textbf{Standard} & \textbf{Confidence} & \textbf{Max} & \textbf{Min} \\ 
  \textbf{(cm)} &  \textbf{(dB)} & \textbf{Deviation (dB)} & \textbf{Interval (dB)} & \textbf{(dB)} & \textbf{(dB)} \\
 \hline
 120 & 3.6403  & 0.0812 & 0.0050  & 3.9  & 3.4 \\  
 140 & 6.2020   & 0.1803 & 0.0112 & 6.7  & 5.1 \\ 
 160 & 9.1434  & 0.2460  & 0.0152 & 9.7  & 8.4 \\ 
 180 & 12.9839 & 0.1278 & 0.0079 & 13.3 & 12.1 \\ 
 200 & 24.2176 & 0.3149 & 0.0195 & 24.9 & 23.2 \\ 
 220 & 15.087  & 0.2635 & 0.0163 & 15.9 & 14.1 \\ 
 240 & 7.6485  & 0.2282 & 0.0141 & 8.2  & 6.8 \\ 
 260 & 4.7130   & 0.2316 & 0.0144 & 5.1  & 2.7 \\ 
 280 & 1.9099  & 0.5534 & 0.0343 & 2.2  & 1.5 \\ 
 \hline
\end{tabular}
\label{table:1}
\end{table}

\begin{table}[ht]
\caption{Statistical analysis of the SNR for the sidelink, at 40 dB transmitter gain.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \textbf{Distance} & \textbf{Average} & \textbf{Standard} & \textbf{Confidence} & \textbf{Max} & \textbf{Min} \\ 
  \textbf{(cm)} &  \textbf{(dB)} & \textbf{Deviation (dB)} & \textbf{Interval (dB)} & \textbf{(dB)} & \textbf{(dB)} \\ 
 \hline
 120 & 12.3448 & 0.3534 & 0.0219 & 13.5 & 11.5 \\  
 140 & 12.6533 & 0.1633 & 0.0101 & 13.2 & 12.0 \\ 
 160 & 19.5281 & 0.2237 & 0.0139 & 20.1 & 18.8 \\ 
 180 & 23.6827 & 0.4287 & 0.0266 & 24.6 & 22.6 \\ 
 200 & 29.2872 & 0.8827 & 0.0547 & 30.7 & 26.8\\ 
 220 & 19.9731 & 0.2355 & 0.0146 & 20.7 & 19.2 \\ 
 240 & 14.9266 & 0.1093 & 0.0068 & 15.2 & 14.6 \\ 
 260 & 8.1482  & 0.1636 & 0.0101 & 8.5  & 7.3 \\ 
 280 & 8.5819  & 0.2286 & 0.0142 & 9.1  & 7.3 \\ 
 \hline
\end{tabular}
\label{table:2}
\end{table}

\begin{table}[ht]
\caption{Statistical analysis of the SNR for the downlink, at 55 dB transmitter gain.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \textbf{Distance} & \textbf{Average} & \textbf{Standard} & \textbf{Confidence} & \textbf{Max} & \textbf{Min} \\ 
  \textbf{(cm)} &  \textbf{(dB)} & \textbf{Deviation (dB)} & \textbf{Interval (dB)} & \textbf{(dB)} & \textbf{(dB)} \\
 \hline
 0   & 31.1044 & 1.5805 & 0.0980  & 34.0   & 27.9 \\  
 20  & 29.8855 & 1.1352 & 0.0704 & 32.2 & 27.2 \\ 
 40  & 28.3759 & 0.7280  & 0.0451 & 29.9 & 26.8 \\ 
 60  & 23.8751 & 1.0637 & 0.0659 & 25.3 & 14.7 \\ 
 80  & 21.3312 & 1.0483 & 0.0650  & 23.1 & 16.4\\ 
 100 & 16.6697 & 1.5552 & 0.0964 & 18.3 & 12.4 \\ 
 120 & 14.8763 & 0.7983 & 0.0495 & 17.3 & 12.6 \\ 
 140 & 13.1189 s& 0.9459 & 0.0586 & 15.5 & 9.0\\ 
 160 & 12.2334 & 0.8596 & 0.0533 & 15.1 & 9.2 \\ 
 180 & 13.2411 & 0.7260  & 0.0450  & 15.2 & 11.0 \\ 
 200 & 11.6577 & 0.8913 & 0.0552 & 13.5 & 9.1 \\ 
 220 & 11.3320  & 0.3551 & 0.0220  & 12.3 & 10.2 \\ 
 240 & 6.0951  & 0.3073 & 0.0190  & 6.9  & 3.2\\
 
 \hline
\end{tabular}
\label{table:3}
\end{table}

\subsection{Throughput measurements and mode selection}

We also measure the maximum throughout using the same experimental setup shown in Fig.~\ref{fig:Results_Scenario} and Fig.~\ref{fig:measurement_setup}. 
In the \ac{3GPP} \ac{LTE} standard, the throughput is determined by the \ac{MCS} index and number of \ac{PRBs} utilized for transmission. We allocate 25 \ac{PRBs} for both downlink and sidelink in our experiment. Therefore, at each measurement location we seek to reach the maximum throughput by increasing the \ac{MCS} index of the transmitters, for the downlink and sidelink, and record the maximum throughput while the observed \ac{BLER} remains at zero. The highest modulation for the downlink is 64 \ac{QAM} and the highest modulation for the sidelink is 16 \ac{QAM} according to the \ac{LTE} standard. Figs.~\ref{fig:Throughput_vs_Distance_40} and~\ref{fig:Throughput_vs_Distance_30} show how the throughput varies according to the position of the remote \ac{UE}; the trends follow closely those reported for the \ac{SNR}.

%Fig.~\ref{fig:Throughput_vs_Distance_40} shows the throughput versus distance for both the sidelink (orange curve) and the downlink (blue curve), with the transmitter gain of the sidelink fixed at 40 dB. From Fig.~\ref{fig:Throughput_vs_Distance_40}, we can see that if the remote \ac{UE} is moved from eNodeB to the cell edge and beyond, the remote \ac{UE} should do downlink till it reaches around 160 cm, after which the throughput through sidelink relay gets better. Therefore at 160 cm the remote \ac{UE} should perform sidelink. After 256 cm, which is the cell edge, the downlink does not work, the remote \ac{UE} has to perform sidelink to get cellular coverage. 

%Fig.~\ref{fig:Throughput_vs_Distance_30} shows the same result with the sidelink transmitter gain at 30 dB. We can see that around 180 cm is the switching point for remote \ac{UE}. We can also see that most of the time throughout for sidelink is low in comparison to throughput when the gain was 40 dB for sidelink. But the throughput is still higher in comparison to downlink, suggesting that remote \ac{UE} should switch to sidelink after 180 cm. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/Throughput_vs_Distance_pic2}  %trim= l b r t
	\caption{Maximum throughput versus distance, for 40 dB sidelink gain.}
    	\label{fig:Throughput_vs_Distance_40}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/Throughput_vs_Distance_pic1}  %trim= l b r t
	\caption{Maximum throughput versus distance for 30 dB sidelink gain.}
    	\label{fig:Throughput_vs_Distance_30}
\end{figure}








==> LTE Standard-Compliant D2D Communication%3A Software-defined Radio Implementation and Evaluation/sections/acro_list.tex <==
\begin{acronym} % Give the longest label here so that the list is nicely aligned

\acro{3GPP}{Third Generation Partnership Project}
\acro{BLER}{Block Error Rate}
\acro{D2D}{Device-to-Device}
\acro{DFT}{Discrete Fourier Transform}
\acro{DSP}{Digital Signal Processing} 
\acro{eWINE}{Elastic Wireless Network Experimentation}
\acro{FDD}{Frequency Division Duplex}
\acro{GUI}{Graphical User Interface}
\acro{IDFT}{Inverse Discrete Fourier Transform}
\acro{LTE}{Long Term Evolution}
\acro{MAC}{Medium Access Control}
\acro{MCS}{Modulation and Coding Scheme}
\acro{MIB}{Master Information Block}
\acro{OFDM}{Orthogonal Frequency Division Multiplexing}
\acro{PDCCH}{Physical Downlink Control Channel}
\acro{PDSCH}{Physical Downlink Shared Channel}
\acro{PHY}{Physical}
\acro{PRBs}{Physical Resource Blocks}
\acro{PSBCH}{Physical Sidelink Broadcast Channel}
\acro{PSCCH}{Physical Sidelink Control Channel}
\acro{PSDCH}{Physical Sidelink Discovery Channel}
\acro{PSS}{Primary Synchronization Signal}
\acro{PSSCH}{Physical Sidelink Shared Channel}
\acro{PSSS}{Primary Sidelink Synchronization Signal}
\acro{QAM}{Quadrature Amplitude Modulation}
\acro{QoS}{quality of service}
\acro{RNTI}{Radio Network Temporary Identifier}
\acro{RSSI}{received signal strength indicator}
\acro{SC-FDMA}{Single Carrier Frequency Division Multiple Access}
\acro{SCI}{Sidelink Control Information}
\acro{SDMA}{Space Division Multiple Access}
\acro{SDN}{Software Defined Networks}
\acro{SDR}{Software-Defined Radio}
\acro{SNR}{Signal-to-Noise Ratio}
\acro{TDMA}{Time Division Multiple Access}
\acro{UE}{User Equipment}
\acro{UHD}{USRP Hardware Driver}
\acro{USRP}{Universal Software Radio Peripheral}


\end{acronym}

==> LTE Standard-Compliant D2D Communication%3A Software-defined Radio Implementation and Evaluation/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we have implemented the first \ac{LTE} standard-compliant \ac{SDR} sidelink \ac{PHY} layer data transmission. We have built a relay \ac{UE} to relay the data received from an eNodeB (through the downlink) to a remote \ac{UE} (through the sidelink). We have also developed functionality for mode selection between infrastructure mode and \ac{D2D} mode on the remote \ac{UE}, providing experimenters with a \ac{GUI} that allows them to perform mode selection and change the radio parameters on the fly. Our measurement results show that the sidelink relay can provide range extension for the cell.
%increase the \ac{SNR} and throughput depending on the geographical distance between eNodeB, relay \ac{UE} and remote \ac{UE}. Through the measurement result we can decide a switching point between sidelink and downlink for better coverage and transmission reliability.

Our ongoing work includes the development of  intelligent mode selection (UE-to-UE versus UE-to-eNodeB) according to network conditions, as well as enhanced \ac{PSCCH} functionality, including user discovery and resource management.


==> LTE Standard-Compliant D2D Communication%3A Software-defined Radio Implementation and Evaluation/sections/introduction.tex <==

\section{Introduction}
\label{sec:introduction}

4G mobile network standards are being extended to support \ac{D2D} communications, functionality that is also expected to be present in 5G~\cite{RSwhitepaper}. Standardization efforts from the \ac{3GPP} are ongoing to provide \ac{LTE} with \ac{D2D} and relaying capabilities, aiming to achieve  coverage extension and improved transmission reliability ~\cite{3GPP}. D2D communication can also support proximity services and public safety use of LTE networks. 
%This type of communication is carried out when two User Equipments (UEs) are close to each other and base station infrastructure is out of reach. 
%D2D communication was initially introduced in \ac{3GPP} standards for use in public safety systems, and is now being extended for commercial cellular communication. 

The \ac{PHY}  communication link between two UEs is referred to as a \emph{sidelink}, standardized in LTE Release 12~\cite{3GPP}, involving user discovery, synchronization, and data transmission. In some locations (e.g. in the edge of cells) where coverage from the \ac{LTE} base station cannot be guaranteed because of low \ac{SNR}, it is possible to use a UE as a relay from the eNodeB to a more remote UE, as illustrated in Fig.~\ref{fig:car_network}. As the user may exhibit mobility and channel conditions change from time to time, dynamic mode selection functionality between infrastructure mode (eNodeB-to-UE) and \ac{D2D} mode (UE-to-UE) is needed.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.4\textwidth, trim = 0mm 0mm 0mm 0mm, clip ]{figures/cars}  %trim= l b r t
	\caption{Sidelink communication in LTE networks.}
	\label{fig:car_network}
\end{figure} 

In this paper we develop the first \ac{SDR} PHY layer sidelink  implementation compliant with the \ac{3GPP} \ac{LTE} standard (Release 12). We also implement functionality to relay data received from an eNodeB (in the downlink) to the remote \ac{UE} (through the sidelink), as well as mode selection functionality to allow the remote UE to switch between sidelink mode and downlink mode according to network conditions.  We extend an open source SDR platform, srsLTE~\cite{srsLTE_link}, with our implementation of the sidelink.
This allows us to dynamically control the radio parameters, e.g. frequency, gain, and \ac{MCS} index. 
We also develop controllers with Graphical User Interfaces (GUIs) that allow experimenters to 
%visualize network connectivity and 
change radio parameter settings on the fly. Our testbed employs the \ac{USRP} platform~\cite{Ettus}. We report measurement results of SNR, throughput and Block Error Rate (BLER) and discuss how these can be used as the criteria for mode selection between direct downlink and relaying through the sidelink. Our implementation of the sidelink, relaying, and mode selection in open source \ac{LTE}  software enables experimentation and prototyping that can assist in standardization, research and development.

D2D communication has been a topic of much recent research, as discussed in the survey~\cite{D2D_survey}. However, only a few research works have developed testbed implementations for testing the performance of systems that rely on \ac{D2D} communications. For instance,
the authors of~\cite{SiChBo2016} present the measurement results of power consumption and \ac{RSSI} for their \ac{D2D} communication in a testbed of sensor nodes following the IEEE 802.15.4 standard. The authors of~\cite{ZhZhZh2016} integrate \ac{D2D} communication and \ac{SDN} by adding \ac{MAC} layer functionality (TDMA, SCMA, etc.) to the basic \ac{OFDM}-based \ac{PHY} layer transmission; the \ac{SDN} controller is then implemented on top of the \ac{MAC} layer protocol. The authors of~\cite{ChLiLi2016} investigate cross-link interference management in a proposed multi-user \ac{D2D} network scenario. The experiment in the paper was carried out by using basic OFDM physical transmission.
However, none of the works mentioned above has produced sidelink implementations that conform to the current 3GPP LTE standardization of D2D communication. To the best of our knowledge, ours is the first PHY layer implementation of D2D communication that is compliant with LTE Release 12 specifications.

% \subsection{Open Source Software Platform}
For implementing the sidelink communication and relay functionality, and to make it compliant with the LTE standard, we have used the srsLTE library~\cite{srsLTE_link}, an open source \ac{PHY} layer platform for software-defined radio implementation of the \ac{FDD} mode of \ac{LTE}~\cite{Gomez-Miguelez2016}. The library follows a modular approach, which helps in combining different PHY layer \ac{DSP} components together without the need to change every element. We have extended the code, implementing the sidelink and relay functionalities while also making use of existing components in srsLTE, namely the uplink and downlink modules, which are compliant to 3GPP LTE Release 8.

%The sponsor of this work, European Commission
This work is conducted in the context of the Horizon 2020 (H2020) \ac{eWINE} project, which focuses on experimental research towards flexible, on-demand end-to-end wireless connectivity. This elastic network connectivity requires the dynamic reallocation of network resources. Our work in this paper implements D2D capabilities in the LTE network which can then be used to dynamically establish a sidelink or a link directly with the eNodeB, depending on current network conditions. 
%The mode selection between infrastructure mode and D2D mode developed in our work can optimize the performance of LTE network links so that mobile users can achieve higher \ac{QoS}. We try to make our current and future work on this open-source D2D communication be a useful reference for future 3GPP standardization activities.










